Analysis of finite-volume discrete adjoint fields for two-dimensional compressible Euler flows

This work deals with a number of questions relative to the discrete and continuous adjoint fields associated with the compressible Euler equations and classical aerodynamic functions. The consistency of the discrete adjoint equations with the corresponding continuous adjoint partial differential equation is one of them. It is has been established or at least discussed only for a handful of numerical schemes and a contribution of this article is to give the adjoint consistency conditions for the 2D Jameson-Schmidt-Turkel scheme in cell-centred finite-volume formulation. The consistency issue is also studied here from a new heuristic point of view by discretizing the continuous adjoint equation for the discrete flow and adjoint fields. Both points of view prove to provide useful information. Besides, it has been often noted that discrete or continuous inviscid lift and drag adjoint exhibit numerical divergence close to the wall and stagnation streamline for a wide range of subsonic and transonic flow conditions. This is analyzed here using the physical source term perturbation method introduced in reference [Giles and Pierce, AIAA Paper 97-1850, 1997]. With this point of view, the fourth physical source term of appears to be the only one responsible for this behavior. It is also demonstrated that the numerical divergence of the adjoint variables corresponds to the response of the flow to the convected increment of stagnation pressure and diminution of entropy created at the source and the resulting change in lift and drag.

==> ALL_REMARKS_ASCII <==


Reviewer #1: I would like to thank the authors for the work in revising the manuscript and the additional computations provided and by the effort in giving point-by-point answers to the questions raised in my previous assessment. The mabnuscript has certainly improved, but there are still some issues that demand clarification. 

I'll begin by addressing your responses to (some of) my previous comments.  Here "Q" refers to my original question, "A" to your answer and "C" to my new comments (if any).


Q: You say in line 435 "that the adjoint RH relations are well satisfied", but that is not quite clear to me from figure 9, so you should probably correct this or make some further comment. Maybe it is well obeyed relative to some reference quantity? Notice that some of the adjoint normal gradients have jumps up to -10 at the shock, while shock equation (41a) for lift has a value of -20 across the shock, where it should be zero.

A: Equation (41a) is now (12a). We are basically plotting the arguments between the brackets in (10) to (12b), not the jump values, so we expect that these quantities remain continuous across the shock but with a value that is not necessarily zero. 

C: OK, thanks, I must have misread your plots! 

Q: Line 531-2: "This relation is not always numerically well satisfied by numerical lift / drag
adjoint fields of Euler flows". I do not know what you mean by this. It is true that the
singularity along the stagnation streamline is not always present, but I am not aware of
any published results challenging the predicted exponent of the divergence. In fact, I think
it would be very interesting that you perform an exponent analysis near the stagnation
streamline (using the source-perturbed flow equations).

A: We referred to numerical experiments by Lozano: figure 12 in the 2017 conference paper and figure 10 in the 2018 AIAA J. article. We performed an exponent analysis close to the wall and a tentative fit with sign(dist)=sqrt(jdistj) law at the stagnation streamline.

C: I see this analysis in Fig A18, but I haven't been able to find a reference to it anywhere in the text. In any case (and this comment is also applicable to the exponent analysis of the adjoints near the wall), this type of analysis is difficult because the structure of the solution is obscured/modified/altered/smoothed out by numerical dissipation (you never actually get to see an infinite value in a numerical simulation), so the exponents could actually depend on the details of numerical dissipation. Have you investigated this possibility?


Q: One of the main conclusions of the paper is that the fourth physical source term is large near walls (and stagnation streamlines) and that causes the observed behavior of the adjoint solutions. I think this observation needs more justification (by independently computing, as stated above, _CL or _CD with the perturbed flow equations) and must address (at least) the following two issues: (1) If _CL or _CD do actually grow as the wall is approached, that may explain why the adjoint solution has large values/gradients near walls. However, this does not explain the observed growth of adjoint values as the mesh is refined. For that, you need to perform a systematic grid convergence study to show that _CL or _CD grow as the mesh is refined.

A: We did this and presented the result in Fig. A20. A growth of dCL4 is observed.

C: I was actually thinking of something like plot A.17 (left) on several meshes, but Fig. A20 is OK. 

Q: (2) If (1) is sorted out, there is still another problem. You claim that the behavior at the wall is the same as at the stagnation streamline. However, for the latter there is some evidence that a true singularity of the adjoint pde exists there. Is there a singularity of the adjoint pde or the adjoint analytic solution at the wall as well? If so, some additional evidence (such as a careful analysis of the behavior of the analytic behavior of ?CL or ?CD, even for potential flow, as in Giles and Pierce 1997 AIAA paper) is required. Or is it an issue of the numerical solution? Notice that if the first possibility is true, then this conflicts with the fact that the adjoint equations require a b.c. at a location where the equations or the solutions) are singular -with infinite values-, which is rather odd.

A: The adjoint is indeed discontinuous across the stagnation streamline with a singular behavior. Though,we were not able to fully explain this singularity, we added some comments at the end of § 5.3.1 that help to clarify the behavior of the adjoint solution: An = nxA + nyB is singular since its eigenvalue vn = 0, so all the components of the adjoint variables cannot be imposed. The same holds with the adjoint derivatives in the normal direction. Finally, let us stress that the singularity no longer holds at the wall as may be observed in Fig. 1: the singular behavior indeed vanishes close the wall and the
adjoint boundary condition (6) is well satisfied.

C: I have several remarks here:
- "An = nxA + nyB is singular since its eigenvalue vn = 0, so all the components of the adjoint variables cannot be imposed. The same holds with the adjoint derivatives in the normal direction." 

An is singular at any streamline, since all streamlines are characteristic lines, so this property alone does not explain the behavior along this particular streamline.

- Page 21 around line 490. Here you derive jump conditions across the stagnation streamline in a rather odd way, using an adjoint \psi_s (such as in shocks) on the stagnation streamline that magically disappears later on. Notice that what you get are essentially the standard jump conditions for 1rst order systems of linear pdes across characteristic lines, A.n[[\psi]] = 0, which are discussed in e.g. Applied Partial Differential Equations Revised Edition 2003 John Ockendon, Sam Howison, Andrew Lacey, and Alexander Movchan. OUPress, chapter 2. 
On the other hand, across the stagnation streamline there appears to be a singularity (with adjoint values diverging at the streamline), not a simple jump, so I am not sure that it makes sense to even write [[\psi]]. 

- Also immediately before line 491, you derive relations between derivatives across the stagnation streamline. However, I believe these are wrong since you are assuming (as in the shock jump conditions) that the tangent derivatives are continuous, which is not granted in this case as it was across shocks since the adjoint variables are not continuous here. Furthermore, if Giles and Pierce are right, adjoint derivatives are also divergent at the stagnation streamline, so again it possibly does not make sense to talk about jumps in derivatives.

- "Finally, let us stress that the singularity no longer holds at the wall as may be observed in Fig. 1: the singular behavior indeed vanishes close the wall and the adjoint boundary condition (6) is well satisfied."

I do not know what you mean by this or what we are expected to see in Fig.1. My question was (and still is) what do we do if there is a mathematical singularity at the wall where adjoint variables are also infinite (as they are expected to be along the stagnation streamline even though this behavior cannot be captured with a numerical solution: you don't see infinite values). In your answer you seem to focus on the point where the stagnation streamline meets the wall. 


Focusing now on the corrected text, there are a few points I would like to mention:

- Page 7, line 161-162: "Let us finally  note that not only the \Lambda components is of physical significance, but also \Lambda\cdot\delta R^d/\epsilon." Please explain why is \Lambda\cdot\delta R^d/\epsilon physically significant . 

- Page13, line 311: "It is is simply."

- Page 15, line 384: "The  percentage of cells with |res| below a threshold is decreasing as the mesh is refined." Shouldn't this be the other way around? The percentage of cells with |res| above a threshold decreases as the mesh is refined

-Page 16, line 386 (and also page 15, line 359). This was also one of my questions in a previous review. "where a perfect adjoint field would exhibit a discontinuity due to the end of the function support)." To me, this is still obscure. The adjoint is actually zero downstream the backward characteristics emanating from the trailing edge simply because of the characteristic structure of the flow: no perturbation downstream those lines can affect the pressure on the airfoil profile and, thus, the lift/drag. Upstream those lines, perturbations can (and do) affect lift/drag, and thus the adjoints take non-zero values. There is thus a simple discontinuity along these characteristic lines (recall that, for linear pdes, jumps are allowed precisely along characteristics) which the numerical solver captures with increased values of the residual, etc. 

- Page 18, line 421-23: "On the contrary, if the source term is located in the subsonic bubble or if one of the three curves enters the subsonic  bubble, then the support of the flow perturbation includes this complete subsonic area in agreement with the elliptic nature of the equations [63, chap. 11]." I am not totally sure about this. I think it depends on the specific residual perturbation. Perturbations 1 and 2 (which are, roughly speaking, a mass source and a vortex) do behave in subsonic regions in the way you suggest . However, enthalpy perturbations (3), on the other hand, only affect the region along the streamline downstream the perturbation point (cf. Giles & Pierce, AIAA 97, page 13, bottom right equation). For the 4th perturbation, the structure is similar (cf equation on page 14 upper right), but here there is the additional effect that the perturbation generates mass sources along the streamline, which do propagate in the way you mention throughout the
subsonic region). 

- Page 22, lines 516-7: "The value of e and the number of iterations have been fixed so that the four first digits of the functions of interest are not altered and the next four or five digits are known after the steady-state iterations." I feel this sentence could use some rewriting. 


- Page 27, line 659 -onwards. Here you discuss the effect of total pressure perturbation focusing on its effect in shock displacement, but the effect in subsonic cases has to be necessarily different. I am aware that this has been discussed elsewhere, but maybe you should clarify this here too.

- Page 27, lines 666-668: "so that our numerical results suggest that the behavior of the adjoint fields in the vicinity of the stagnation streamline (where the authors of [1] predicted a numerical divergence under simplifying assumptions) and in the vicinity of the wall are identical." 
You have indeed given evidence linking the behavior along the wall and the stagnation streamline. However, I am still worried that the adjoint diverges at the wall but the adjoint is required to obey a boundary condition. 



Reviewer #2: The authors have addressed the comments raised in the first review.  The writing has also improved, although there are still some mistakes, mostly extra commas and a few usage/word-choice errors.
